Joint Behavior and Common Belief

For over 25 years, common belief has been widely viewed as necessary for joint behavior. But this is not quite correct. We show by example that what can naturally be thought of as joint behavior can occur without common belief. We then present two variants of common belief that can lead to joint behavior, even without standard common belief ever being achieved, and show that one of them, action-stamped common belief, is in a sense necessary and sufficient for joint behavior. These observations are significant because, as is well known, common belief is quite difficult to achieve in practice, whereas these variants are more easily achievable.

==> eptcsdata.tex <==
\providecommand{\firstpage}{221}
\providecommand{\publicationstatus}{R. Verbrugge (Ed.): Theoretical Aspects of \\
Rationality and Knowledge 2023 (TARK 2023)\\
EPTCS 379, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.379.18}{10.4204/EPTCS.379.18}}
\pdfoutput=1

